The Effect of Communication Topology on Scalar Field Estimation by Networked Robotic Swarms

This paper studies the problem of reconstructing a two-dimensional scalar field using a swarm of networked robots with local communication capabilities. We consider the communication network of the robots to form either a chain or a grid topology. We formulate the reconstruction problem as an optimization problem that is constrained by first-order linear dynamics on a large, interconnected system. To solve this problem, we employ an optimization-based scheme that uses a gradient-based method with an analytical computation of the gradient. In addition, we derive bounds on the trace of observability Gramian of the system, which helps us to quantify and compare the estimation capability of chain and grid networks. A comparison based on a performance measure related to the H2 norm of the system is also used to study robustness of the network topologies. Our resultsare validated using both simulated scalar fields and actual ocean salinity data.

==> latex files/Macros.tex <==



% Ordered and Unordered
\newcommand{\unord}[1]{t'_{#1}}
\newcommand{\ord}[1]{t_{#1}}
\newcommand{\rad}{\delta}
\newcommand{\dia}{2\delta}
\newcommand{\nor}{n}
\newcommand{\sat}{d}
\newcommand{\psat} {p_{sat}}
\newcommand{\satint}{[0,\sat]}

\newcommand{\leftint}[1]{L_{#1}}
\newcommand{\rightint}[1]{R_{#1}}
\newcommand{\inter}[1]{I_{#1}}
\newcommand{\perm}{p}
\newcommand{\unwrap}{U}

\newcommand{\real}{\mathbb{R}}

\newcommand{\prob}{\mathcal{P}}

% Curve and unit interval
\newcommand{\curve}{\gamma} %{\mathcal{C}}
\newcommand{\uint}{\mathcal{I}}
\newcommand{\sint} {\mathcal{S}}
\newcommand{\clength}{l}

% Event space and Event simplex
\newcommand{\espace}{\Omega}
\newcommand{\efav}{\mathcal{E}}



% Measure of event
\newcommand{\meas}[1]{|#1|}

% Slacks
\newcommand{\sla}{s}
\newcommand{\sli}[1]{s_{#1}}  %{\mathcal{S}} %{s_{#1}}
\newcommand{\slset}{S}
\newcommand{\rsli}[1]{s'_{#1}}
\newcommand{\slx}[1]{S_{#1}}
\newcommand{\slaset}{ \{ \slx{i} \} }
\newcommand{\slasetop} { S_m}

% Initial and Final angles
\newcommand{\ordinit}{\ord{1}}
\newcommand{\ordfinal}{\ord{n}}
\newcommand{\ordseq} { \langle t_1,t_2,\ldots,t_n \rangle}

\newcommand{\fint}[1]{F_{#1}}  %\mathcal{F}_{#1}}

% Simplex and hypercube

\newcommand{\simp} {\mathcal{S}}
\newcommand{\hyp}{\mathcal{H}}
\newcommand{\simpn}[1]{{S}_{#1}}  %{\simp _{#1}}
\newcommand{\redsimpn}[2]{\simpn{#1}(#2)}
\newcommand{\hypn}[1]{{H}_{#1}}  %{\mathcal{H}_{#1}}
\newcommand{\simhypn}[1]{E_{#1}} %{\mathcal{SH}_{#1}}
\newcommand{\Sum}{\Sigma}
\newcommand{\sladom}{D}

% Outside points
\newcommand{\simpoutn}[1]{{E}'_{#1}} %{\mathcal{SH}'_{#1}}
\newcommand{\simpoutnk}[2]{{E}'_{#1}(#2)} %{\mathcal{SH}'_{#1}(#2)}
\newcommand{\unchanged}{U}  %{\mathcal{U}}
\newcommand{\augmented}{A_{k}} %{\mathcal{A}}


\newcommand{\ujoint}{f_u}
\newcommand{\ojoint}{f}

% Beta density
\newcommand{\B}[2]{B(#1,#2)}
\newcommand{\po}[3]{{#1}^{#2}{(1-#1)}^{#3}}
\newcommand{\bet}[3]{\mathrm{Beta}(#1|#2,#3)} 
\newcommand{\ibet}[3]{\mathrm{I}(#1|#2,#3)}
% Probability density function, distribution function
%\newcommand{\todo}[1]{#1}
\newcommand{\ind}[1]{\mathbf{1}_#1}

\newcommand{\NP}{\mathsf{NP}}
\newcommand{\NPH}{\mathsf{NP-HARD}}

==> latex files/preamble.tex <==
% Upper-case    A B C D E F G H I J K L M N O P Q R S T U V W X Y Z
% Lower-case    a b c d e f g h i j k l m n o p q r s t u v w x y z
% Digits        0 1 2 3 4 5 6 7 8 9
% Exclamation   !           Double quote "          Hash (number) #
% Dollar        $           Percent      %          Ampersand     &
% Acute accent  '           Left paren   (          Right paren   )
% Asterisk      *           Plus         +          Comma         ,
% Minus         -           Point        .          Solidus       /
% Colon         :           Semicolon    ;          Less than     <
% Equals        =           Greater than >          Question mark ?
% At            @           Left bracket [          Backslash     \
% Right bracket ]           Circumflex   ^          Underscore    _
% Grave accent  `           Left brace   {          Vertical bar  |
% Right brace   }           Tilde        ~

% Make \title integrate PDF title and bookmark and build \thetitle
\let\oldtitle\title
\renewcommand\title[1]{%
    \begingroup
        \providecommand{\ttlit}{}%
        \renewcommand{\ttlit}[1]{}%
        \providecommand{\titlenote}{}%
        \renewcommand{\titlenote}[1]{}%
        \hypersetup{pdftitle={#1}}%
        \def\thetitle{#1}%
        \pdfbookmark[0]{#1}{title}
    \endgroup
    \oldtitle{#1}%
}

% Give us a \mykeywords
\newcommand\mykeywords[1]{%
    \begingroup
        \providecommand{\and}{}%
        \renewcommand{\and}{\unskip, }%
        \hypersetup{pdfkeywords={#1}}%
        \xdef\thekeywords{#1.}%
    \endgroup}

% Give us a \myauthors
\newcommand\myauthors[1]{%
    \begingroup
        \providecommand{\and}{}%
        \renewcommand{\and}{\unskip, }%
        \hypersetup{pdfauthor={#1}}%
        \xdef\theauthors{#1}%
    \endgroup}

% Use calc so we can do length math during definitions
\usepackage{calc}

% extdash gives us dashes that don't break hyphenation
\usepackage[shortcuts]{extdash}

% Graphics support
\usepackage{graphicx}

% Better tabular support
\usepackage{booktabs}

\usepackage{verbatim}

\usepackage{amsmath}
\usepackage{psfrag}

%----------------------------------------------------------------------|

%%fakepart{Setup and configure references}
%----------------------------------------------------------------------|

% ACM says that abbrv is fine
% (is compress OK?)

% Unfortunately, natbib does not TIE textual references to their
% citations. So authors sometimes get separated from citations when they
% come at the end of the line. The following lines attempt to fix this
% problem.
%
% The lines below do the equivalent of . . .
%
%       \renewcommand\citet[1]{\citeauthor{#1}~\citep{#1}}
%
% but they handle the star and capitalization and optional argument
% cases too.
\makeatletter
%
%%% These lines test for star and number of arguments and call the
%%% workhorses below
%
% Test for star (mid-sentence and start-sentence forms)
\def\citet{\@ifstar{\citetstar}{\citetnostar}}
\def\Citet{\@ifstar{\Citetstar}{\Citetnostar}}
%
% No star found. Now test for argument count.
\def\citetnostar{\@ifnextchar[{\squarecitet}{\simplecitet}}
\def\squarecitet[#1]{\@ifnextchar[{\twocitet[#1]}{\onecitet[#1]}}
\def\Citetnostar{\@ifnextchar[{\squareCitet}{\simpleCitet}}
\def\squareCitet[#1]{\@ifnextchar[{\twoCitet[#1]}{\oneCitet[#1]}}
%
% Star found. Now test for argument count.
\def\citetstar{\@ifnextchar[{\squarecitetstar}{\simplecitetstar}}
\def\squarecitetstar[#1]{\@ifnextchar[{\twocitetstar[#1]}{\onecitetstar[#1]}}
\def\Citetstar{\@ifnextchar[{\squareCitetstar}{\simpleCitetstar}}
\def\squareCitetstar[#1]{\@ifnextchar[{\twoCitetstar[#1]}{\oneCitetstar[#1]}}
%
\makeatother
%
%
%%% The following actually do the \cite work
%
% The \citet cases (no arg, one arg, and two args)
\def\simplecitet#1{\citeauthor{#1}~\citep{#1}}
\def\onecitet[#1]#2{\citeauthor{#2}~\citep[#1]{#2}}
\def\twocitet[#1][#2]#3{\citeauthor{#3}~\citep[#1][#2]{#3}}
%
% The \citet* cases (no arg, one arg, and two args)
\def\simplecitetstar#1{\citeauthor*{#1}~\citep{#1}}
\def\onecitetstar[#1]#2{\citeauthor*{#2}~\citep[#1]{#2}}
\def\twocitetstar[#1][#2]#3{\citeauthor*{#3}~\citep[#1][#2]{#3}}
%
% The \Citet cases (no arg, one arg, and two args)
\def\simpleCitet#1{\Citeauthor{#1}~\citep{#1}}
\def\oneCitet[#1]#2{\Citeauthor{#2}~\citep[#1]{#2}}
\def\twoCitet[#1][#2]#3{\Citeauthor{#3}~\citep[#1][#2]{#3}}
%
% The \Citet* cases (no arg, one arg, and two args)
\def\simpleCitetstar#1{\Citeauthor*{#1}~\citep{#1}}
\def\oneCitetstar[#1]#2{\Citeauthor*{#2}~\citep[#1]{#2}}
\def\twoCitetstar[#1][#2]#3{\Citeauthor*{#3}~\citep[#1][#2]{#3}}
%----------------------------------------------------------------------|

%%fakepart{Setup for math}
%----------------------------------------------------------------------|
\usepackage[cmex10]{mathtools}             % Loads and extends amsmath
\interdisplaylinepenalty=2500              % (automatically break within
                                           % multiline equations (cmex10
                                           % too))
\usepackage{amsfonts,amssymb}
\usepackage{mathrsfs}                      % Gives us \mathscr for \setset

%----------------------------------------------------------------------|

%%fakepart{Setup autoreferencing}
%----------------------------------------------------------------------|

\usepackage{varioref}
\labelformat{subfigure}{\thefigure\textup{(#1)}}
\labelformat{equation}{\textup{(#1)}}
%\labelformat{enumi}{\textup{(#1)}}

% Hyperref is not just about links...
\usepackage[%
        pagebackref=false,
        bookmarks=true,bookmarksopen=true,
        bookmarksnumbered=true,
        breaklinks=true,
        colorlinks=true,
        anchorcolor=blue,citecolor=blue,
        urlcolor=blue,linkcolor=blue,filecolor=blue,
        menucolor=blue,
        %pdfpagelabels=true,hypertexnames=false,
        %plainpages=false,
    ]{hyperref}
% Gives us a \url that breaks
%\usepackage{url}
\usepackage{breakurl}
% Give us a \doi that links
\usepackage{doi}
\def\doitext{doi:~}

% Prefer to use package subfig instead, but use old subfigure for
% technical reasons.
\usepackage{subfigure}

% Fixes a problem with how old versions of hyperref record item labels
\makeatletter
\@ifpackageloaded{hyperref}{%
\@ifpackageloaded{amsmath}{%
\newcommand{\AMShreffix}[1]{%
        \expandafter\let\csname AMShreffix#1\expandafter\endcsname%
                \csname #1\endcsname%
        \expandafter\renewcommand\csname #1\endcsname{%
                \@hyper@itemfalse\csname AMShreffix#1\endcsname}}
\AtBeginDocument{%
\AMShreffix{equation}
\AMShreffix{align}
\AMShreffix{alignat}
\AMShreffix{flalign}
\AMShreffix{gather}
\AMShreffix{multline}
}}{}}{}
\makeatother

% Need to redefine \autoref. Should use abbreviations inside the
% sentence and full names at the beginning of sentences. Additionally,
% need to handle the plural cases.

\def\subfigureautorefname{\figureautorefname}
\def\subfloatautorefname{\figureautorefname}
%
\def\subsectionautorefname{\sectionautorefname}
\def\subsubsectionautorefname{\sectionautorefname}
%
\def\subappendixautorefname{\appendixautorefname}
\def\subsubappendixautorefname{\appendixautorefname}
\def\appendixparagraphautorefname{\appendixautorefname}

% Use Fig.
\def\figurename{Fig.}



%----------------------------------------------------------------------|

%%fakepart{Custom macros}
%----------------------------------------------------------------------|
%\InputIfFileExists{Macros.tex}{}{}
%----------------------------------------------------------------------|


==> preamble.tex <==
% Upper-case    A B C D E F G H I J K L M N O P Q R S T U V W X Y Z
% Lower-case    a b c d e f g h i j k l m n o p q r s t u v w x y z
% Digits        0 1 2 3 4 5 6 7 8 9
% Exclamation   !           Double quote "          Hash (number) #
% Dollar        $           Percent      %          Ampersand     &
% Acute accent  '           Left paren   (          Right paren   )
% Asterisk      *           Plus         +          Comma         ,
% Minus         -           Point        .          Solidus       /
% Colon         :           Semicolon    ;          Less than     <
% Equals        =           Greater than >          Question mark ?
% At            @           Left bracket [          Backslash     \
% Right bracket ]           Circumflex   ^          Underscore    _
% Grave accent  `           Left brace   {          Vertical bar  |
% Right brace   }           Tilde        ~

% Make \title integrate PDF title and bookmark and build \thetitle
\let\oldtitle\title
\renewcommand\title[1]{%
    \begingroup
        \providecommand{\ttlit}{}%
        \renewcommand{\ttlit}[1]{}%
        \providecommand{\titlenote}{}%
        \renewcommand{\titlenote}[1]{}%
        \hypersetup{pdftitle={#1}}%
        \def\thetitle{#1}%
        \pdfbookmark[0]{#1}{title}
    \endgroup
    \oldtitle{#1}%
}

% Give us a \mykeywords
\newcommand\mykeywords[1]{%
    \begingroup
        \providecommand{\and}{}%
        \renewcommand{\and}{\unskip, }%
        \hypersetup{pdfkeywords={#1}}%
        \xdef\thekeywords{#1.}%
    \endgroup}

% Give us a \myauthors
\newcommand\myauthors[1]{%
    \begingroup
        \providecommand{\and}{}%
        \renewcommand{\and}{\unskip, }%
        \hypersetup{pdfauthor={#1}}%
        \xdef\theauthors{#1}%
    \endgroup}

% Use calc so we can do length math during definitions
\usepackage{calc}

% extdash gives us dashes that don't break hyphenation
\usepackage[shortcuts]{extdash}

% Graphics support
\usepackage{graphicx}

% Better tabular support
\usepackage{booktabs}

\usepackage{verbatim}

\usepackage{amsmath}
\usepackage{psfrag}

%----------------------------------------------------------------------|

%%fakepart{Setup and configure references}
%----------------------------------------------------------------------|

% ACM says that abbrv is fine
% (is compress OK?)

% Unfortunately, natbib does not TIE textual references to their
% citations. So authors sometimes get separated from citations when they
% come at the end of the line. The following lines attempt to fix this
% problem.
%
% The lines below do the equivalent of . . .
%
%       \renewcommand\citet[1]{\citeauthor{#1}~\citep{#1}}
%
% but they handle the star and capitalization and optional argument
% cases too.
\makeatletter
%
%%% These lines test for star and number of arguments and call the
%%% workhorses below
%
% Test for star (mid-sentence and start-sentence forms)
\def\citet{\@ifstar{\citetstar}{\citetnostar}}
\def\Citet{\@ifstar{\Citetstar}{\Citetnostar}}
%
% No star found. Now test for argument count.
\def\citetnostar{\@ifnextchar[{\squarecitet}{\simplecitet}}
\def\squarecitet[#1]{\@ifnextchar[{\twocitet[#1]}{\onecitet[#1]}}
\def\Citetnostar{\@ifnextchar[{\squareCitet}{\simpleCitet}}
\def\squareCitet[#1]{\@ifnextchar[{\twoCitet[#1]}{\oneCitet[#1]}}
%
% Star found. Now test for argument count.
\def\citetstar{\@ifnextchar[{\squarecitetstar}{\simplecitetstar}}
\def\squarecitetstar[#1]{\@ifnextchar[{\twocitetstar[#1]}{\onecitetstar[#1]}}
\def\Citetstar{\@ifnextchar[{\squareCitetstar}{\simpleCitetstar}}
\def\squareCitetstar[#1]{\@ifnextchar[{\twoCitetstar[#1]}{\oneCitetstar[#1]}}
%
\makeatother
%
%
%%% The following actually do the \cite work
%
% The \citet cases (no arg, one arg, and two args)
\def\simplecitet#1{\citeauthor{#1}~\citep{#1}}
\def\onecitet[#1]#2{\citeauthor{#2}~\citep[#1]{#2}}
\def\twocitet[#1][#2]#3{\citeauthor{#3}~\citep[#1][#2]{#3}}
%
% The \citet* cases (no arg, one arg, and two args)
\def\simplecitetstar#1{\citeauthor*{#1}~\citep{#1}}
\def\onecitetstar[#1]#2{\citeauthor*{#2}~\citep[#1]{#2}}
\def\twocitetstar[#1][#2]#3{\citeauthor*{#3}~\citep[#1][#2]{#3}}
%
% The \Citet cases (no arg, one arg, and two args)
\def\simpleCitet#1{\Citeauthor{#1}~\citep{#1}}
\def\oneCitet[#1]#2{\Citeauthor{#2}~\citep[#1]{#2}}
\def\twoCitet[#1][#2]#3{\Citeauthor{#3}~\citep[#1][#2]{#3}}
%
% The \Citet* cases (no arg, one arg, and two args)
\def\simpleCitetstar#1{\Citeauthor*{#1}~\citep{#1}}
\def\oneCitetstar[#1]#2{\Citeauthor*{#2}~\citep[#1]{#2}}
\def\twoCitetstar[#1][#2]#3{\Citeauthor*{#3}~\citep[#1][#2]{#3}}
%----------------------------------------------------------------------|

%%fakepart{Setup for math}
%----------------------------------------------------------------------|
\usepackage[cmex10]{mathtools}             % Loads and extends amsmath
\interdisplaylinepenalty=2500              % (automatically break within
                                           % multiline equations (cmex10
                                           % too))
\usepackage{amsfonts,amssymb}
\usepackage{mathrsfs}                      % Gives us \mathscr for \setset

%----------------------------------------------------------------------|

%%fakepart{Setup autoreferencing}
%----------------------------------------------------------------------|

\usepackage{varioref}
\labelformat{subfigure}{\thefigure\textup{(#1)}}
\labelformat{equation}{\textup{(#1)}}
%\labelformat{enumi}{\textup{(#1)}}

% Hyperref is not just about links...
\usepackage[%
        pagebackref=false,
        bookmarks=true,bookmarksopen=true,
        bookmarksnumbered=true,
        breaklinks=true,
        colorlinks=true,
        anchorcolor=blue,citecolor=blue,
        urlcolor=blue,linkcolor=blue,filecolor=blue,
        menucolor=blue,
        %pdfpagelabels=true,hypertexnames=false,
        %plainpages=false,
    ]{hyperref}
% Gives us a \url that breaks
%\usepackage{url}
\usepackage{breakurl}
% Give us a \doi that links
\usepackage{doi}
\def\doitext{doi:~}

% Prefer to use package subfig instead, but use old subfigure for
% technical reasons.
\usepackage{subfigure}

% Fixes a problem with how old versions of hyperref record item labels
\makeatletter
\@ifpackageloaded{hyperref}{%
\@ifpackageloaded{amsmath}{%
\newcommand{\AMShreffix}[1]{%
        \expandafter\let\csname AMShreffix#1\expandafter\endcsname%
                \csname #1\endcsname%
        \expandafter\renewcommand\csname #1\endcsname{%
                \@hyper@itemfalse\csname AMShreffix#1\endcsname}}
\AtBeginDocument{%
\AMShreffix{equation}
\AMShreffix{align}
\AMShreffix{alignat}
\AMShreffix{flalign}
\AMShreffix{gather}
\AMShreffix{multline}
}}{}}{}
\makeatother

% Need to redefine \autoref. Should use abbreviations inside the
% sentence and full names at the beginning of sentences. Additionally,
% need to handle the plural cases.

\def\subfigureautorefname{\figureautorefname}
\def\subfloatautorefname{\figureautorefname}
%
\def\subsectionautorefname{\sectionautorefname}
\def\subsubsectionautorefname{\sectionautorefname}
%
\def\subappendixautorefname{\appendixautorefname}
\def\subsubappendixautorefname{\appendixautorefname}
\def\appendixparagraphautorefname{\appendixautorefname}

% Use Fig.
\def\figurename{Fig.}



%----------------------------------------------------------------------|

%%fakepart{Custom macros}
%----------------------------------------------------------------------|
%\InputIfFileExists{Macros.tex}{}{}
%----------------------------------------------------------------------|

